StyTr$^2$: Image Style Transfer with Transformers

The goal of image style transfer is to render an image with artistic features guided by a style reference while maintaining the original content. Owing to the locality in convolutional neural networks (CNNs), extracting and maintaining the global information of input images is difficult. Therefore, traditional neural style transfer methods face biased content representation. To address this critical issue, we take long-range dependencies of input images into account for image style transfer by proposing a transformer-based approach called StyTr$^2$. In contrast with visual transformers for other vision tasks, StyTr$^2$ contains two different transformer encoders to generate domain-specific sequences for content and style, respectively. Following the encoders, a multi-layer transformer decoder is adopted to stylize the content sequence according to the style sequence. We also analyze the deficiency of existing positional encoding methods and propose the content-aware positional encoding (CAPE), which is scale-invariant and more suitable for image style transfer tasks. Qualitative and quantitative experiments demonstrate the effectiveness of the proposed StyTr$^2$ compared with state-of-the-art CNN-based and flow-based approaches. Code and models are available at https://github.com/diyiiyiii/StyTR-2.

==> Figs/fig_artflow.tex <==
\begin{figure}%[t]
\setlength{\abovecaptionskip}{0mm}
\centering
\includegraphics[width= 0.98\linewidth]{image/artflow}
\caption{Comparisons of model robustness with ArtFlow.
}
\label{fig:artflow}
\end{figure}


==> Figs/fig_compare.tex <==
\newcommand\comparisonfigurewidth{0.118}

\begin{figure*}%[t]
%\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/c1.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/s1.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/ours1.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/atta1.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/artflow1.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/mcc1.png}
% \includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/dfp1.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/aams1.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/adain1.png}

\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/c10.png}
\includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/s10.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/ours10.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/atta10.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/artflow10.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/mcc10.png}
% \includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/dfp3.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/aams10.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/adain10.png}

\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/c11.png}
\includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/s11.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/ours11.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/atta11.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/artflow11.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/mcc11.png}
% \includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/dfp6.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/aams11.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/adain11.png}

\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/c12.png}
\includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/s12.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/ours12.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/atta12.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/artflow12.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/mcc12.png}
% \includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/dfp7.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/aams12.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/adain12.png}

\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/c9.png}
\includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/s9.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/ours9.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/atta9.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/artflow9.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/mcc9.png}
% \includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/dfp7.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/aams9.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/adain9.png}

\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/c8.png}
\includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/s8.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/ours8.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/atta8.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/artflow8.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/mcc8.png}
% \includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/dfp7.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/aams8.png}
\includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/adain8.png}

\includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/c16.png}
\includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/s16.png}
\includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/ours16.png}
\includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/atta16.png}
\includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/artflow16.png}
\includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/mcc16.png}
% \includegraphics[width=\comparisonfigurewidth\linewidth]{image/figs_comparisons/dfp7.png}
\includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/aams16.png}
\includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/adain16.png}

\vspace{-2pt}
\begin{minipage}{\comparisonfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\comparisonfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\comparisonfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\comparisonfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\comparisonfigurewidth\linewidth}
    \centering
    \figtext{ArtFlow}
\end{minipage}
\begin{minipage}{\comparisonfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\comparisonfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\comparisonfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}
%\includegraphics[width= \linewidth]{image/compare}
\vspace{-7pt}
\caption{Comparisons of style transfer results using different methods. % The first column shows content images, the second column shows style images. The remaining columns are stylized results generated by different methods.
}
%\vspace{-2mm}
\label{fig:compare}
\end{figure*}


==> Figs/fig_limitation.tex <==
\begin{figure}[h]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width= \linewidth]{image/bad_case.pdf}
\caption{Limitation of our StyTr$^2$ framework.
}
\label{fig:bad_case}
\end{figure}

==> Figs/fig_net_compare.tex <==
\begin{figure*}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\textwidth]{image/net_compare.pdf}
\caption{A comparison of encoder-transfer-decoder style transfer structure and our structure.
The CNN-based method could lead to biased style transfer, while the transformer-based method could avoid feature leak and achieve unbiased style transfer. 
}
% \vspace{-4mm}
\label{fig:net_compare}
\end{figure*}


==> Figs/fig_pipline.tex <==
\begin{figure*}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width= \textwidth]{image/pipline.pdf}
\caption{
Comparisons of intermediate layers using the rightmost image as both the content and the style image in a reconstruction task.
% (a) Our method. We decode the features extracted in the first three layers of our transformer decoder.
% The reconstruction results maintain distinct structures with increasing detailed brushstrokes.
% Since transformer can obtain long-range dependencies, the results generated by each layer look visually promising.
% (b) The CNN-based method proposed by Gatys et al.~\cite{gatys:2016:image}. We reconstruct the input image from from layers $conv1\_1$, $ \{ conv1\_1, conv2\_1 \}$, $\{conv1\_1, conv2\_1, conv3\_1, conv4\_1\}$ of a pretrained VGG network.
(a) Image reconstruction results from layers $conv1\_1$, $ \{ conv1\_1, conv2\_1 \}$, $\{conv1\_1, conv2\_1, conv3\_1, conv4\_1\}$ of a pretrained VGG network based on Gatys et al.~\cite{gatys:2016:image}.
(b) Feature visualizations of three layers of the transformer decoder.
% We find that reconstruction results match the style of a given image on an increasing scale as the network deepens.
% Different layers of CNN-based model focus on different scale information, thus it cannot generate satisfactory result by every layer.
}

\label{fig:pipline}
\end{figure*}


==> Figs/fig_progressive.tex <==
\begin{figure*}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width= \textwidth]{image/progressive}
\caption{The influence of progressive generation of transformer decoder.
}
% \vspace{-4mm}
\label{fig:progressive}
\end{figure*}


==> Figs/fig_sup1.tex <==
\newcommand\supfigurewidth{0.196}
\newcommand\supfigurespace{-5pt}
\begin{figure*}%[t]
%\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow1.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{ArtFlow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc1.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain1.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c2.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours2.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta2.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow2.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s2.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc2.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams2.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain2.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c3.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours3.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta3.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow3.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s3.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc3.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams3.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain3.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

% \begin{minipage}{\supfigurewidth\linewidth}
%     \centering
%     \figtext{Content}
% \end{minipage}
% \begin{minipage}{\supfigurewidth\linewidth}
%     \centering
%     \figtext{Style}
% \end{minipage}
% \begin{minipage}{\supfigurewidth\linewidth}
%     \centering
%     \figtext{Ours}
% \end{minipage}
% \begin{minipage}{\supfigurewidth\linewidth}
%     \centering
%     \figtext{AdaAttN}
% \end{minipage}
% \begin{minipage}{\supfigurewidth\linewidth}
%     \centering
%     \figtext{ArtFlow}
% \end{minipage}
% \begin{minipage}{\supfigurewidth\linewidth}
%     \centering
%     \figtext{MCC}
% \end{minipage}
% \begin{minipage}{\supfigurewidth\linewidth}
%     \centering
%     \figtext{AAMS}
% \end{minipage}
% \begin{minipage}{\supfigurewidth\linewidth}
%     \centering
%     \figtext{AdaIN}
% \end{minipage}
%\includegraphics[width= \linewidth]{image/compare}
\vspace{-7pt}
\caption{Comparisons of style transfer results using different methods.
% The first column shows content images, the second column shows style images. The remaining columns are stylized results generated by different methods.
}\label{fig:sup1}
\end{figure*}


==> Figs/fig_sup2.tex <==
\begin{figure*}%[t]
%\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c4.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours4.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta4.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow4.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s4.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc4.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams4.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain4.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c5.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours5.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta5.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow5.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s5.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc5.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams5.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain5.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c6.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours6.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta6.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow6.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s6.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc6.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams6.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain6.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

% \begin{minipage}{\supfigurewidth\linewidth}
%     \centering
%     \figtext{Content}
% \end{minipage}
% \begin{minipage}{\supfigurewidth\linewidth}
%     \centering
%     \figtext{Style}
% \end{minipage}
% \begin{minipage}{\supfigurewidth\linewidth}
%     \centering
%     \figtext{Ours}
% \end{minipage}
% \begin{minipage}{\supfigurewidth\linewidth}
%     \centering
%     \figtext{AdaAttN}
% \end{minipage}
% \begin{minipage}{\supfigurewidth\linewidth}
%     \centering
%     \figtext{ArtFlow}
% \end{minipage}
% \begin{minipage}{\supfigurewidth\linewidth}
%     \centering
%     \figtext{MCC}
% \end{minipage}
% \begin{minipage}{\supfigurewidth\linewidth}
%     \centering
%     \figtext{AAMS}
% \end{minipage}
% \begin{minipage}{\supfigurewidth\linewidth}
%     \centering
%     \figtext{AdaIN}
% \end{minipage}
%\includegraphics[width= \linewidth]{image/compare}
\vspace{-7pt}
\caption{Comparisons of style transfer results using different methods. 
% The first column shows content images, the second column shows style images. The remaining columns are stylized results generated by different methods.
}
%\vspace{-2mm}
\label{fig:sup2}
\end{figure*}

==> Figs/fig_sup3.tex <==
\begin{figure*}%[t]
%\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c7.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours7.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta7.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow7.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s7.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc7.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams7.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain7.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c8.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours8.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta8.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow8.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}


\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s8.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc8.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams8.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain8.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c9.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours9.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta9.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow9.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s9.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc9.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams9.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain9.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\vspace{-7pt}
\caption{Comparisons of style transfer results using different methods.
% The first column shows content images, the second column shows style images. The remaining columns are stylized results generated by different methods.
}
%\vspace{-2mm}
\label{fig:sup3}
\end{figure*}


==> Figs/fig_sup4.tex <==
\begin{figure*}%[t]
%\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c10.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours10.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta10.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow10.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s10.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc10.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams10.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain10.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c11.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours11.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta11.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow11.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s11.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc11.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams11.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain11.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c12.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours12.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta12.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow12.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s12.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc12.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams12.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain12.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\vspace{-7pt}
\caption{Comparisons of style transfer results using different methods.
% The first column shows content images, the second column shows style images. The remaining columns are stylized results generated by different methods.
}
%\vspace{-2mm}
\label{fig:sup4}
\end{figure*}

==> Figs/fig_supp_ItoS.tex <==
% \begin{figure}%[!ht]
% \setlength{\abovecaptionskip}{2mm}
% \centering
% \includegraphics[width= \linewidth]{image/ItoS2.pdf}
% \caption{Comparisons of CNN and Linear projection through several rounds of image stylization.
% }
% \label{fig:ItoS2}
% \end{figure}


\newcommand\Ttosfigurewidth{0.22}
\newcommand\Ttostextwidth{0.015}
% \newcommand\nTtostextwidth{0.007}

\begin{figure}%[b]
\setlength{\abovecaptionskip}{2mm}
\centering

\begin{minipage}{\Ttostextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Style}}
\end{minipage}
\hspace{0pt}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/s.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/l1.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/l2.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/l3.png}
\end{minipage}
\begin{minipage}{\Ttostextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Linear}}
\end{minipage}

\begin{minipage}{\Ttostextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Content}}
\end{minipage}
\hspace{0pt}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/c.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/cnn1.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/cnn2.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/cnn3.png}
\end{minipage}
\begin{minipage}{\Ttostextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{CNN}}
\end{minipage}

\begin{minipage}{\Ttosfigurewidth\linewidth}
    \centering
    \figtext{Input}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \centering
    \figtext{Round 1}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \centering
    \figtext{Round 2}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \centering
    \figtext{Round 3}
\end{minipage}
\caption{Comparisons of CNN based and our linear projection based layers through several rounds of image stylization.
}
\vspace{-2mm}
\label{fig:ItoS2}
\end{figure}

==> Figs/fig_supp_big.tex <==
\newcommand\bigfigurewidth{0.31}

\begin{figure*}%[t]
%\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/c1.png}
\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/r1.png}
\includegraphics[width=\bigfigurewidth\linewidth,height=\bigfigurewidth\linewidth]{image/figs_bigs/s1.png}


\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/c2.png}
\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/r2.png}
\includegraphics[width=\bigfigurewidth\linewidth,height=\bigfigurewidth\linewidth]{image/figs_bigs/s2.png}

\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/c3.png}
\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/r3.png}
\includegraphics[width=\bigfigurewidth\linewidth,height=\bigfigurewidth\linewidth]{image/figs_bigs/s3.png}

\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/c4.png}
\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/r4.png}
\includegraphics[width=\bigfigurewidth\linewidth,height=\bigfigurewidth\linewidth]{image/figs_bigs/s4.png}

\vspace{-2pt}
\begin{minipage}{\bigfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\bigfigurewidth\linewidth}
    \centering
    \figtext{Our results}
\end{minipage}
\begin{minipage}{\bigfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\vspace{-7pt}
\caption{More style transfer results in a large resolution of $768 \times 768$.
% The first column shows content images, the second column shows style images. The remaining columns are stylized results generated by different methods.
}\label{fig:big}
\end{figure*}


==> Figs/fig_supp_noise.tex <==
\begin{figure*}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\textwidth]{image/noise}
\caption{Comparisons of model robustness with ArtFlow. We visualize the impact of adding a small perturbation $\Delta$ following a Gaussian distribution on the stylized images in the \engordnumber{4} and \engordnumber{7} columns.
}
\label{fig:noise}
\end{figure*}


==> Figs/fig_supp_progressive.tex <==
\newcommand\pecomparisonfigurewidth{0.24}

\begin{figure}%[b]
\setlength{\abovecaptionskip}{2mm}
\centering
%\includegraphics[width=\linewidth]{image/pure_position.pdf}
\includegraphics[width=\pecomparisonfigurewidth\linewidth,height=\pecomparisonfigurewidth\linewidth]{image/figs_progressive/c.PNG}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{image/figs_progressive/single.PNG}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{image/figs_progressive/m.PNG}
\includegraphics[width=\pecomparisonfigurewidth\linewidth,height=\pecomparisonfigurewidth\linewidth]{image/figs_progressive/s.PNG}
% \includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/s9.png}

\begin{minipage}{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{Single-layer}
\end{minipage}
\begin{minipage}{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{Multi-layer}
\end{minipage}
\begin{minipage}{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}

\caption{The impact of progressive generation of transformer decoder.
}\label{fig:progressive}
\end{figure}


==> Figs/fig_supp_weights.tex <==
% \begin{figure}%[!h]
% \setlength{\abovecaptionskip}{0mm}
% \centering
% \includegraphics[width= \linewidth]{image/weight.pdf}
% \caption{Impact of style weight.
% }
% \label{fig:weight}
% \end{figure}

\newcommand\weightfigurewidth{0.24}

\begin{figure}%[b]
\setlength{\abovecaptionskip}{2mm}
\centering
%\includegraphics[width=\linewidth]{image/pure_position.pdf}
\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/c1.png}
\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/wl1.png}
\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/wh1.png}
\includegraphics[width=\weightfigurewidth\linewidth,height=\pecomparisonfigurewidth\linewidth]{image/figs_weight/s1.png}
% \includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/s9.png}

\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/c2.png}
\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/wl2.png}
\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/wh2.png}
\includegraphics[width=\weightfigurewidth\linewidth,height=\pecomparisonfigurewidth\linewidth]{image/figs_weight/s2.png}

\begin{minipage}{\weightfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\weightfigurewidth\linewidth}
    \centering
    \figtext{$\lambda_{s} = 5$}
\end{minipage}
\begin{minipage}{\weightfigurewidth\linewidth}
    \centering
    \figtext{$\lambda_{s} = 10$}
\end{minipage}
\begin{minipage}{\weightfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\caption{Impact of style weight.
}
\vspace{-2mm}
\label{fig:weight}
\end{figure}


==> Figs/fig_teaser.tex <==
%\begin{figure*}[t]
%\setlength{\abovecaptionskip}{2mm}
%\centering
%\includegraphics[width=\linewidth]{image/intermediate_layers.pdf}
%\caption{
%Comparisons of intermediate layers using the rightmost image as both the content and the style image in a reconstruction task.
% (a) Our method. We decode the features extracted in the first three layers of our transformer decoder.
% The reconstruction results maintain distinct structures with increasing detailed brushstrokes.
% Since transformer can obtain long-range dependencies, the results generated by each layer look visually promising.
% (b) The CNN-based method proposed by Gatys et al.~\cite{gatys:2016:image}. We reconstruct the input image from from layers $conv1\_1$, $ \{ conv1\_1, conv2\_1 \}$, $\{conv1\_1, conv2\_1, conv3\_1, conv4\_1\}$ of a pretrained VGG network.
%(a) Image reconstruction results from layers $conv1\_1$, $ \{ conv1\_1, conv2\_1 \}$, $\{conv1\_1, conv2\_1, conv3\_1, conv4\_1\}$ of a pretrained VGG network based on Gatys et al.~\cite{gatys:2016:image}.
%(b) Feature visualizations of three layers of the transformer decoder.
% We find that reconstruction results match the style of a given image on an increasing scale as the network deepens.
% Different layers of CNN-based model focus on different scale information, thus it cannot generate satisfactory result by every layer.
%}
%\label{fig:pipline}
%\end{figure*}


\begin{center}
    \centering
    \captionsetup{type=figure}
\includegraphics[width=0.8 \linewidth]{image/teaser.pdf}
\caption{
Our stylization results. Our method can generate promising stylized effect with well-preserved content structures and fine details.
}
\label{fig:teaser}
\end{center}

==> Figs/fig_user_study.tex <==
\begin{table*}%[!h]
\small
% \setlength\tabcolsep{9.5pt}
\centering
\begin{floatrow}

\capbtabbox{
\begin{tabular}{m{1.1cm}<{\centering}|m{0.7cm}<{\centering}m{0.5cm}<{\centering}m{0.5cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}}
\toprule
&ArtFlow&MCC&DFP& AAMS& AdaIN \\
\midrule
% Num. & 783&820&827&809&734 \\
votes &25.7&25.5&22.6&18.2& 23.5\\
% Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
\bottomrule
\end{tabular}
}{
% \vspace{-2mm}
\caption{User study results. }
% \vspace{-2mm}
\label{tab:user}
    }
\capbtabbox{
\begin{tabular}{m{1.1cm}<{\centering}|m{0.7cm}<{\centering}m{0.5cm}<{\centering}m{0.5cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}}
\toprule
&ArtFlow&MCC&DFP& AAMS& AdaIN \\
\midrule
% Num. & 783&820&827&809&734 \\
votes &25.7&25.5&22.6&18.2& 23.5\\
% Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
\bottomrule
\end{tabular}
}{
% \vspace{-2mm}
\caption{User study results. }
% \vspace{-2mm}
\label{tab:user}
    }
\capbtabbox{
\begin{tabular}{m{1.1cm}<{\centering}|m{0.7cm}<{\centering}m{0.5cm}<{\centering}m{0.5cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}}
\toprule
&ArtFlow&MCC&DFP& AAMS& AdaIN \\
\midrule
% Num. & 783&820&827&809&734 \\
votes &25.7&25.5&22.6&18.2& 23.5\\
% Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
\bottomrule
\end{tabular}
}{
% \vspace{-2mm}
\caption{User study results. }
% \vspace{-2mm}
\label{tab:user}
    }
\end{floatrow}
\vspace{-4mm}
\end{table*}

==> Figs/fig_vit.tex <==
\newcommand\vitfigurewidth{0.32}

\begin{figure}%[t]
%\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\vitfigurewidth\linewidth]{image/figs_vits/c1.png}
\includegraphics[width=\vitfigurewidth\linewidth]{image/figs_vits/r1.png}
\includegraphics[width=\vitfigurewidth\linewidth,height=\vitfigurewidth\linewidth]{image/figs_vits/s1.png}

\includegraphics[width=\vitfigurewidth\linewidth]{image/figs_vits/c2.png}
\includegraphics[width=\vitfigurewidth\linewidth]{image/figs_vits/r2.png}
\includegraphics[width=\vitfigurewidth\linewidth,height=\vitfigurewidth\linewidth]{image/figs_vits/s2.png}

\vspace{-5pt}
\begin{minipage}{\vitfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\vitfigurewidth\linewidth}
    \centering
    \figtext{VIT}
\end{minipage}
\begin{minipage}{\vitfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\vspace{-7pt}
\caption{Style transfer results using model trained by VIT-based loss. 
% The first column shows content images, the second column shows style images. The remaining columns are stylized results generated by different methods.
}
%\vspace{-2mm}
\label{fig:vit}
\end{figure}


==> Sections/checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{ We present some bad cases and analyze the reason in the Appendix.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{ This work is proposed for promising painting creation using referenced content and style images. Although the application of this technique can not threaten to personal safety, deep fake could be used by crooks. }
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section~\ref{sec:Method}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Section~\ref{sec:Method}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{ We include the source code in the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section 4.1 }
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{ See the supplemental material.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See the supplemental material.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{ We describe the instructions detailly to ensure fairness and effectiveness of the experiment.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNo{ Our user study does not have potential participant risks.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{ We invited 100 participants to conduct our user study, and pay them each $20$ RMB. }
\end{enumerate}

\end{enumerate}


==> Tables/Quantity_comparison.tex <==
\begin{table*}%[!h]
\small
% \setlength\tabcolsep{9.5pt}
\centering
\begin{floatrow}
\capbtabbox{
\begin{tabular}{p{0.5cm}<{\centering}|p{0.5cm}<{\centering} p{0.7cm}<{\centering} p{0.5cm}<{\centering} p{0.5cm}<{\centering} p{0.6cm}<{\centering} p{0.6cm}<{\centering} }
\toprule
$\downarrow$&Ours&ArtFlow&MCC&DFP& AAMS& AdaIN \\
\midrule
$\contentloss$   & \textbf{1.91}&2.13&2.38&2.67&2.44& 2.34 \\
$\styleloss$ &\textbf{1.47}&3.08&1.56&2.12& 3.18& 1.91 \\
% Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
\bottomrule
\end{tabular}
}{
%\vspace{-2mm}
\caption{Quantitative comparisons.}
%\vspace{-2mm}
\label{tab:loss}
}
\capbtabbox{
\begin{tabular}{m{1.1cm}<{\centering}|m{0.7cm}<{\centering}m{0.5cm}<{\centering}m{0.5cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}}
\toprule
&ArtFlow&MCC&DFP& AAMS& AdaIN \\
\midrule
% Num. & 783&820&827&809&734 \\
rates of votes &25.7&25.5&22.6&18.2& 23.5\\
% Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
\bottomrule
\end{tabular}
}{
% \vspace{-2mm}
\caption{User study results. }
% \vspace{-2mm}
\label{tab:user}
    }
\end{floatrow}
\vspace{-4mm}
\end{table*}






==> Tables/tab_supp_progressive.tex <==
\begin{table}%[!h]
\small
\setlength\tabcolsep{2.5pt}
\centering
\begin{tabular}{c|cc}
\toprule
&Single-layer &Ours (multi-layer)  \\
\midrule
$\contentloss$ $\downarrow$ & 1.94& \textbf{1.91} \\
$\styleloss$ $\downarrow$ & 2.38 & \textbf{1.47}  \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{Quantitative evaluation of progressive generation.}
\label{tab:loss1}
\end{table}


==> packages.tex <==
%%%%%%%%% PAPER TYPE  - PLEASE UPDATE FOR FINAL VERSION
%\usepackage[review]{cvpr}      % To produce the REVIEW version
\usepackage{cvpr}              % To produce the CAMERA-READY version
%\usepackage[pagenumbers]{cvpr} % To force page numbers, e.g. for an arXiv version
\newcommand{\final}{1}
% Include other packages here, before hyperref.
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{floatrow}
\usepackage{makecell}
\usepackage{engord}
%\newfloatcommand{capbtabbox}{table}
%\floatsetup[table]{capposition=top}
\usepackage{adjustbox}
\usepackage{enumitem}

% It is strongly recommended to use hyperref, especially for the review version.
% hyperref with option pagebackref eases the reviewers' job.
% Please disable hyperref *only* if you encounter grave issues, e.g. with the
% file validation for the camera-ready version.
%
% If you comment hyperref and then uncomment it, you should delete
% ReviewTempalte.aux before re-running LaTeX.
% (Or just hit 'q' on the first LaTeX run, let it finish, and you
%  should be clear).
\usepackage[pagebackref,breaklinks,colorlinks]{hyperref}

% Support for easy cross-referencing
\usepackage[capitalize]{cleveref}

